Explaining the Uncertain: Stochastic Shapley Values for Gaussian Process Models

We present a novel approach for explaining Gaussian processes (GPs) that can utilize the full analytical covariance structure present in GPs. Our method is based on the popular solution concept of Shapley values extended to stochastic cooperative games, resulting in explanations that are random variables. The GP explanations generated using our approach satisfy similar favorable axioms to standard Shapley values and possess a tractable covariance function across features and data observations. This covariance allows for quantifying explanation uncertainties and studying the statistical dependencies between explanations. We further extend our framework to the problem of predictive explanation, and propose a Shapley prior over the explanation function to predict Shapley values for new data based on previously computed ones. Our extensive illustrations demonstrate the effectiveness of the proposed approach.

==> sections/00_discuss.tex <==
\section{Brainstorm and Discussion}

\paragraph{What is the motivation?} 
\begin{itemize}
    \item There is no GP specific SHAP algorithm, i.e. estimation of the cooperative game does not use any characteristic of GPs.
    \item Näive application of KernelSHAP~\citep{lundberg2017unified} to GP posterior mean will discard the useful uncertainty information.
    \item Advance approach either 
    \begin{enumerate}
        \item incorporate an interpretable part while building the GP model for regression~\citep{yoshikawa_gaussian_2021}
        \item sample multiple functions and explain each of them simultaneously, then you get an uncertainty of the prediction.~\citep{marx_but_nodate}
    \end{enumerate}
    The former approach cannot be applied to GP models beyond regression and also require substantial modification. The latter approach uses sampling approach but do not take into account GP specific characteristic to estimate the value functions. RKHS-SHAP cannot be applied näively to samples from a GP, therefore they still need to run KernelSHAP.
\end{itemize}

\paragraph{What are some existing literature on the topic of uncertainty and Shapley values?}
\begin{enumerate}
    \item Bayesian Shapley values~\citep{slack_reliable_nodate} formulate the weighted least square approach from \cite{lundberg2017unified} as a Bayesian weighted linear regression and compute the posterior of the Shapley values to get uncertainty. \Alan{It is useful to think about the source of uncertainty the Bayesian Shapley values are representing - I think BayesSHAP encapsulate epistemic uncertainty when computing the Shapley values. In our case, we kind of want to reflect the uncertainty from our epistemic uncertainty from GP instead. (of course can combine the two approach but nothing special at all then)}
    \item Uncertainty Shapley values~\citep{gao_uncertain_2017} is quite a relevant piece of work to ours. They consider the scenario where the payoff of the cooperative game follows an uncertain distribution~\citep{liu2010uncertainty}\footnote{A more sophisticated way to model uncertainty that subsume probability theory.} They then define the expected Shapley value and an $\alpha$-optimistic Shapley value, which with no surprise, are obtained by defining the cooperative game as the expectation and $\alpha$ level quantile of the underlying uncertain distribution. \Alan{There are suprisingly few literature on probabilistic games but quite a few on uncertain games.. I guess the latter do subsume the former. I don't know but this will be a great connection back to the literature and say GP actually induces to an uncertain game which we can quantify its distribution (for regression) or estimate its moments (for non-regression). }
    \item Variance and Standard deviation game~\citep{galeotti_comparison_2021,colini-baldeschi_variance_2018}: These are problems defined in finance where they have $n$ instruments $X_{1:n}$ and a coalition is $S_J = \sum_{j\in J}X_j$. Since these instruments could be correlated, it is unclear how to allocate the total variance $\VV(\sum_j X_j)$ to each instrument. Shapley value is then applied. 
    \item \cite{fryer_shapley_2020} consider decomposing the coefficient of determination $R^2$ and attribute them to the covariates using Shapley values. Since $R^2$ measures the variance explained by features, this paper has some conceptual similarity to our work because we also want to attribute the variance of our grand coalition $\VV_f[\EE_X[f(X)\mid X_S=x_S]]$ to our variables. 
\end{enumerate}

\paragraph{How do we formulate this problem?}
\begin{enumerate}
    \item Gaussian process induces a cooperative game with probabilistic outcomes, i.e. for $f\sim \cG\cP $
    \begin{align}
        \nu_{x, f}(S) = \EE_X[f(X)\mid X_S=x_S]
    \end{align}
    is a random variable. In standard GP regression, we know this quantity can be formulated as a conditional mean process with estimable mean and covariance structure. If now there is $g(x) = t\circ f (x)$ where $t$ is some transformation, then we can still estimate the mean and variance of the corresponding probabilistic value function
    \begin{align}
        \nu'_{x, g}(S) = \EE_X[t\circ f(X) \mid X_S=x_S]
    \end{align}
    using Taylor approximations where the terms in the approximation can be estimated using CMEs and Covariance operator. \Alan{Dino please see if it make sense? can discuss in meeting}
    \item When given a probabilistic game, one could construct different cooperative games based on this probability distribution, for example,
    \begin{enumerate}
        \item The mean game: $^m\nu_{x, f}(S) := \EE_f\EE_X[f(X) \mid X_S=x_S]$ which leads to RKHS-SHAP.
        \item The variance game: $^v\nu_{x, f}(S) := \VV_f\EE_X[f(X)\mid X_S=x_S]$ which leads to a distribution of uncertainty to each feature that follows the Shapley axioms: sum to total variance, symmetric covariates get the same variance portion, null features contain no variance. \Alan{It is worth discussing how to interpret this variance credit. It is not as straightforward as saying it is the uncertainty of the estimation of the usual Shapley values.}
        \item the quantile game: $^q\nu_{x, f}(S)$ but not sure how informative this would be.
    \end{enumerate}
    % \item Another perspective that could be used to justify this variance credit as some kind of uncertainty is the following argument: Recall in LIME~\citep{lime}, one places a surrogate linear model around the decision boundary of a specific data point $x$, sample pseudo observations $x'$ based on some weights $w$ and solve the linear regression problem, and the coefficients of that model is the attribution. In \cite{lundberg2017unified}, they showed that Shapley values can be obtained using a similar argument under a specific choice of $w$. Basically, they were asking ``if I assign a number to each feature and add them up, how to do that
    \item \textbf{Moment Matching Perspective:} Another perspective to reason why the allocated variance scores can be seen as the variance of Shapley values is as follows: SVs are numbers that add up to the grand coalition that satisfy fairness axioms. Can we generalise such axioms to distribution level? i.e. Assuming normality for the attribution, since now the grand coalition is a Gaussian, can we say we want to add those shapley distributions add such that it equates to the grand total? and since grand total is Gaussian, we want to match mean and variance? 
\end{enumerate}

\paragraph{Can we motivate this axiomatically?} Let's say we start by listing what are the natural extensions of the deterministic Shapley axioms to probabilistic axioms: Denote $\nu: 2^\Omega \to \cP$ the probabilistic cooperative game, $\phi_i$ the now probabilistic Shapley value, then ideally the following seems natural
\Dino{these are written in terms of distributional equality of these random variables, 2-4 in terms of their marginal distributions, so not clear if the dependence structure can vary and still satisfy axioms? Hence r.v. equality might need to be stronger and need to be defined in terms of equality of the actual mappings that determine random variables? Or is efficiency actually sufficient to determine joint distribution of $\phi_i$...?}
\begin{enumerate}
    \item P-Efficient: $\PP(\sum \phi_i) = \PP(\nu(\Omega))$
    \item P-Symmetry: If $i, j$ are probabilistic exchangeable, i.e. $\PP(\nu(S\cup i)) = \PP(\nu(S\cup j)) ~\forall S\subseteq \Omega\backslash \{i,j\}$, then 
    \begin{align}
        \PP(\phi_i) = \PP(\phi_j)
    \end{align}
    \item P-Null Player: If $\PP(\nu(S\cup i)) = \PP(\nu(S))~\forall S\subseteq \Omega\backslash \{i\}$, then $\phi_i = 0$ 
    \item P-linear: For ``independent'' game $\nu, \omega$, i.e. $\forall S\subset \Omega, \nu(S), \omega(S)$ are independent, we define the sum of the probabilistic game as $(\nu + \omega)(S) = \nu(S) + \omega(S)$, then $\PP(\phi(\nu + \omega)) = \PP(\phi(\nu)) + \PP(\phi(\omega))$
\end{enumerate}

\begin{proposition}
For the Gaussian cooperative game, the only independent Gaussian Shapley distribution that satisfies the above axioms are the ones where mean and variance are decomposed separately from the mean game and variance game. 
\end{proposition}

\begin{proof}
If we construct the independent Gaussians based on decomposing mean game and variance game, then we satisfy P-Efficiency, P-Symmetry, P-Null, and P-linear. Uniqueness is by inductive logic, mean and variance game decomposition give unique values, therefore the Gaussians constructed based on these quantities are therefore unique.
\end{proof}

\hrule
\subsection{Can we formulate the game itself as a GP on $S$ as well?}

Everything above didn't explicitly trying to model the covariance across coalition. We now show that this is actually possible, or more correctly, estimable,
\begin{proposition}
    $\nu_f(x, S) := \EE_X[f(X) \mid X_S=x_S]$ can be formulated as a GP with the following covariance structure $\kappa: \left(\cX\times 2^\Omega\right)^2 \to \RR$:
    \begin{align}
        \kappa\left((x, S), (x', S')\right)
        &=Cov\left(\nu_f(x, S), \nu_f(x', S')\right) \\ 
        &= \iiiint f(X)f'(X') d\PP(X\mid X_S=x_S) d\PP(X'\mid X'_{S'} = x_{S'}') df df' \\
        &= \iint {\bar k}(X, X') d\PP(X\mid X_S=x_S) d\PP(X'\mid X'_{S'} = x_{S'}') \\
\intertext{where in particular for standard GP regression, ${\bar k}(x, x') = k(x, x') - k(x,X) (K_{XX} + \lambda I)^{-1}k(X,x')$, we can use conditional mean embeddings to estimate this covariance structure.}
        &= \mu_{X\mid X_S=x_S}^\top \mu_{X\mid X_{S'}=x_{S'}} - \text{ugly terms}
    \end{align}
\end{proposition}

\subsection{Actually, let's start from scratch.}

Now let's think: we can fully model the covariance structure (and mean) of the cooperative game. Can we speed up computation of Shapley values? Before that, let's rethink the whole pipeline and what we want to achieve:
\begin{enumerate}
    \item If the game gives a probabilistic outcome, what is the right notion of credit allocation now? If we want to satisfy \textbf{P-Efficient}, \textbf{P-Symmetric}, \textbf{P-Null}, and \textbf{P-linear}, is the classical solution applied to random games still correct? Lets call them P-SVs for now.
    \begin{align}
        \phi_i^P(\nu) = \sum_{S\subseteq \Omega \backslash {i}} c_{|S|} \left(\nu(S\cup i) - \nu(S)\right)
    \end{align}
    \Dino{this basically seems to be all we need, see below}
 
 Write   
\[
\phi_{i}=\sum_{S}c_{|S|}\left(\nu\left(S\cup i\right)-\nu\left(S\right)\right)
\]
By linearity, expectation of this random variable is just the usual Shapley value. And for the variance, we write
\begin{eqnarray*}
\text{Var}\left[\phi_{i}\right] & = & \sum_{S}\sum_{S'}c_{|S|}c_{|S'|}\text{Cov}\left(\nu\left(S\cup i\right)-\nu\left(S\right),\nu\left(S'\cup i\right)-\nu\left(S'\right)\right)\\
 & = & \sum_{S}\sum_{S'}c_{|S|}c_{|S'|}\left\langle \mu_{X|X_{S}=x_{S},X_{i}=x_{i}}-\mu_{X|X_{S}=x_{S}},\mu_{X|X_{S'}=x_{S'},X_{i}=x_{i}}-\mu_{X|X_{S'}=x_{S'}}\right\rangle \\
 & = & \left\langle \sum_{S}c_{|S|}\left(\mu_{X|X_{S}=x_{S},X_{i}=x_{i}}-\mu_{X|X_{S}=x_{S}}\right),\sum_{S'}c_{|S'|}\left(\mu_{X|X_{S'}=x_{S'},X_{i}=x_{i}}-\mu_{X|X_{S'}=x_{S'}}\right)\right\rangle \\
 & = & \left\Vert \sum_{S}c_{|S|}\left(\mu_{X|X_{S}=x_{S},X_{i}=x_{i}}-\mu_{X|X_{S}=x_{S}}\right)\right\Vert ^{2},
\end{eqnarray*}
so variance is just the RKHS norm of the Shapley representer (With respect to the posterior kernel).
    \Alan{This random quantity seems to still satisfy these axioms. Need to check P-linear, but the others seem trivial.}
    \item Now I need to show that the same weighted least square regression solution from \cite{lundberg2017unified} still give rise to the P-SVs, i.e. let $Z$ be the matrix of all possible binary vectors of length $d$ with $2^d$ rows and $d$ columns. The $P-SVs$ can be computed as:
    \begin{align}
        \phi^P = (Z^\top W Z)^{-1}Z^\top \bfv
    \end{align}
    where $\bfv = [\nu(z_i)]_{i=1}^{2^d}$. Apologise for notation abuse but please interpret $S_i$ as the features that are activated in $z_i$. \Alan{This statement should still hold because the original proof is just a bunch of linear operations}
    \item Now focus on the case of GP, where we know $\bfv$ is simply a vector of Gaussian random variable, therefore $\phi^P$ will be a Gaussian random variable with the following structure: denote $A = (Z^\top W Z)^{-1}Z^\top$
    \begin{align}
        \phi^P \sim N(A\EE[\bfv], A\VV[\bfv]A^\top)
    \end{align}
    \item We have used the fact our games are Gaussian random variable, but we haven't really used the fact they are Gaussian processes, let's think a bit more:
    \begin{align}
        
    \end{align}
\end{enumerate}

==> sections/98_depreciatedshapley_prior.tex <==
% \section{Predictive explanation}
% \label{sec: shapley_prior}

% The key idea behind the GP-SHAP algorithm is that Gaussian processes remains tractable under conditional expectations~(to build the s-game) and linear operations~(to compute the SSVs). Leveraging these properties, we move beyond explaining GPs and apply this framework to more general predictive models by formulating explanations as multi-output GPs. By doing this, we can estimate a predictive uncertainty for explanations generated using non-GP models and furthermore, predict explanations for previously unseen data.

% In the following, we abuse notations and denote $\phi: \cX \to \RR^d$ as the explanation function that return feature attributions. We present the prior over $\phi$ induced by positing a $\cG\cP(0, k)$ prior over $f$,
% \begin{proposition}[The Shapley prior over $\phi$] Given $f\sim \cG\cP(0, k)$ and the stochastic game $\nu_f(\bfx, S) = \EE[f(X)\mid X_S=\bfx_S]$, they induce a multi-output GP prior over the explanation functions $\phi \sim \cG\cP(0, \kappa)$, where $\kappa: \cX \times \cX \to \RR^{d \times d}$ is the matrix-valued covariance kernel of the form,
% \begin{align}
%     \kappa(\bfx, \bfx') = A \Xi[\bfx, \bfx'] A^\top, \quad \Xi[\bfx, \bfx'] = \left\{\EE[k(X, X') \mid X_{S_i}=\bfx_{S_i}, X'_{S_j}=\bfx'_{S_j}]\right\}_{i,j = 1}^{2^d, 2^d}.
% \end{align}
% \end{proposition}
% With this prior over explanations in place, we can treat explanations obtained from a variety of models, such as trees, deep neural networks, or RKHS functions, as a realization from this prior and build a predictive model based on these explanations. This approach is based on the assumption that there exists a true data generation mechanism $f_*: \cX\to\cY$, and any model $f$ we use, is an approximation of $f_*$, therefore any explanations we obtain for $f$ are also considered attempts to reveal explanations under $f_*$. This perspective has also been adopted by \citet{chen2020true} and \citet{marx_but_nodate}. One could now then treat the explanations as labels, fit a multi-output GP regression and optimise for the hyperparameters, and construct a predictive model as follow: 
% \begin{proposition}[Predictive explanations] Given a dataset $\bfD_\phi = \{(\bfx_i, \bfphi_i)\}_{i=1}^n = (\bfX, \bfPhi_\bfX)$ where $\bfphi_i\in\RR^d$ are the computed Shapley values under some predictive model $f$ and $\bfPhi_\bfX = [\bfphi_1,...,\bfphi_n]^\top$, the predictive explanations for new data $\bfx'$ is distributed as,
% \begin{align}
%     \phi(\bfx')\mid \bfD_\phi \sim \cN\left(b_\kappa(\bfx', \bfX)^\top\operatorname{vec}(\Phi_\bfX), \quad \kappa(\bfx',\bfx') - \kappa(\bfx', \bfX)b_\kappa(\bfx', \bfX)\right)
% \end{align}
% where $b_\kappa(\bfx', \bfX) := (\hkappa_{\bfX\bfX} + \sigma_\phi^2 I)^{-1}\kappa(\bfX, \bfx)$, $\hkappa_{\bfX\bfX}$ is the gram matrix for kernel $\kappa$ of size $nd \times nd$, $\kappa(\bfx',\bfX) = [\kappa(\bfx', \bfx_1),...,\kappa(\bfx', \bfx_n)]$ is of size $d \times nd$ and $\sigma^2_\phi$ is the noise parameter for regression.
% \end{proposition}

% % \subsection{Universality of the multi-task Shapley kernel}

% % \begin{defn}[multi-task Shapley kernel] We define the multi-task Shapley kernel as $\kappa: \cX\times \cX \to \RR^{d\times d}$ taking the form
% % \begin{align}
% %     \kappa(\bfx, \bfx') = A\Xi(\bfx)^\top \Xi(\bfx') A^\top ,
% % \end{align}
% % where $\Xi(\bfx) =  [\EE[k(X, \cdot) \mid X_{S_1}=\bfx_{S_1}], \ldots, \EE[k(X, \cdot) \mid X_{S_{2^d}}=\bfx_{S_{2^d}}]]$ and the corresponding RKHS $\cH_\kappa$ is constructed as $\{ A\Xi(\cdot)^\top f, \quad \forall f\in \cH_k \}$, \Alan{Is this true?... Does it make sense to say I construct such an RKHS from $\cH_k$? what is the reasoning...}
% % \end{defn}

% % \begin{restatable}[Universality of $\kappa$ in $C_{Sh}(\cX, \Upphi)$]{theorem}{kappauniversality}
% %  Denote $\Upphi = (\RR^d, ||\cdot ||_1)$. If $k$ is universal in $C_0(\cX, \RR)$, the space of bounded real-valued continuous functions, then $\kappa$ is universal in $C_{Sh}(\cX, \Upphi)$, the space of $\Upphi$-valued continuous functions of the form,
% % \begin{align}
% %     C_{Sh}(\cX, \Upphi) = \left\{\phi_f(\cdot) = A[\EE[f(X)\mid X_{S_1} = \cdot], ..., \EE[f(X)\mid X_{S_{2^d}} = \cdot]]^\top \quad \forall f\in C_0(\cX) \right\}
% % \end{align}    
% % \end{restatable}

% % \begin{theorem} Denote $\Upphi = (\RR^d, ||\cdot ||_1)$ as the Banach target space, and $C_0^d(\cX, \Upphi)$ the Banach space of continuous $\Upphi-$valued continuous function on a compact subset of $\cX$ with the supremum norm, where the functions take the following form,
% % \begin{align}
% % C_0^d(\cX, \Upphi):= \left\{ \phi(\cdot) = A[\EE[f(X)\mid X_{S_1} = \cdot], ..., \EE[f(X)\mid X_{S_{2^d}} = \cdot]]^\top \quad \forall f\in C_0(\cX)\right\}
% % \end{align}


% % \subsection{Universality of the Shapley kernel}
% % We perform analysis on the expressiveness of our Shapley kernel by proving its universality in the space of deterministic Shapley values. We focus on the analysis of $\phi_i:\cX \to \RR$, the explanation function that give Shapley values for feature $i$. Denote $C^0(\cX)$ as the space of bounded continuous real-valued function on $\cX$, and define the space of Shapley values of feature $i$ induced from $C_0(\cX)$ as,
% % \begin{align*}
% %     \Phi_i(\cX) := \left\{\phi_{i, f}(\cdot) = \sum_{S\subseteq [d] \backslash \{i\}} c_{|S|} \EE[f(X) \mid X_{S\cup i} = \cdot] - \EE[f(X)\mid X_S = \cdot], \forall f \in C^0(\cX) \right\}
% % \end{align*}
% % then we have the following result,
% % \begin{theorem}[Universality of $\kappa_i$ in $\Phi_i(\cX)$] If our kernel $k$ is universal with respect to $C^0(\cX)$, the Shapley kernel for the $i^{th}$ player is defined as $\kappa_i(\bfx, \bfx') = \Psi_{i}(\bfx)^\top \Psi_{i}(\bfx')$ where $\Psi_i(\bfx)$ is the following feature map,
% % \begin{align}
% %     \Psi_i(\bfx) = \sum_{S\subseteq [d]\backslash\{i\}} c_{|S|} \left[\EE[k(\cdot, X)\mid X_{S\cup i} = \bfx_{S\cup i}] - \EE[k(\cdot, X)\mid X_{S} = \bfx_{S}]\right] 
% % \end{align}
% % then the corresponding RKHS $\cH_{\kappa_i}$ is dense with respect to the space of Shapley values for feature $i$.
% % \end{theorem}
% % This results demonstrates the expressiveness of our proposed kernel and it basically means that for any explanation generated from bounded continuous function $f$, there exists some function in $\cH_{\kappa_i}$ that is arbitrarily close to it given enough data.


% % \section{Simple illustrations}

% % \subsection{1D Regression Case} 

% % We first consider a simple $1D$ regression problem:
% % \begin{itemize}
% %     \item We first sample $X\sim N(0,1)$ and set $Y = X * sin(2\pi X) + N(0, 0.1)$
% %     \item Fit a GP with Matern Kernel
% %     \item Run GP-SHAP and plot the mean and variance of Shapley values together along with $X$.
% % \end{itemize}
% % We see that from~Fig\ref{fig:1d_reg}, GP-SHAP are very certain that prediction with large uncertainty gives 0 contribution. \textcolor{red}{I somewhat feel like there are too many factors coming into play here, so I wouldn't be 100 per cent trust the result yet. Need rechecking.}
% % \begin{figure}
% %     \centering
% %     \includegraphics[width=\textwidth]{figure/1-D_GPR_vs_GPSHAP.png}
% %     \caption{1D regression plot for both the GP and GPSHAP. We see that GP-SHAP are very certain that the OOD points are not contributing (SV=0).}
% %     \label{fig:1d_reg}
% % \end{figure}

% % \subsection{Redundant feature case with $10$ features}
% % We now consider a multivariate prediction problem:
% % \begin{itemize}
% %     \item Sample $X\sim N(0, I_10)$ and set $Y = X_1\sin(2\pi \frac{1}{9}\sum_{j=1}^9 X_j) + N(0, 0.1)$. Therefore, the last feature is completely redundant.
% %     \item Fit a GP with Matern Kernel
% %     \item Run GP-SHAP
% % \end{itemize}
% % We summarise the results using a bar plot and beeswarm plot over both the mean and std of the Shapley values in Fig~\ref{fig:redundant_exp_10_feature_mean} and Fig.~\ref{fig:redundant_exp_10_feature_std}. In particular, we see that not only our GP can identify the 10th feature as being much more useless compared to the others, it is more certain about this explanation as shown by the lower average uncertainty on the 10th featuere.
% % \begin{figure}
% %      \centering
% %      \begin{subfigure}[b]{0.4\textwidth}
% %          \centering
% %          \includegraphics[width=\textwidth]{figure/redundant_feature_exp_10_feature/GPSHAP_Mean_Barplot.png}
% %          \caption{GP-SHAP Mean Bar plot}
% %      \end{subfigure}
% %      \hfill
% %      \begin{subfigure}[b]{0.48\textwidth}
% %          \centering
% %          \includegraphics[width=\textwidth]{figure/redundant_feature_exp_10_feature/GPSHAP_Mean_BeeSwarm.png}
% %          \caption{GP-SHAP Mean Beeswarm plot}
% %          \label{fig:three sin x}
% %      \end{subfigure}
% %     \caption{Examining the mean of GP-SHAP values.}
% %     \label{fig:redundant_exp_10_feature_mean}
% % \end{figure}

% % \begin{figure}
% %      \centering
% %      \begin{subfigure}[b]{0.4\textwidth}
% %          \centering
% %          \includegraphics[width=\textwidth]{figure/redundant_feature_exp_10_feature/GPSHAP_std_Barplot.png}
% %          \caption{GP-SHAP STD Bar plot}
% %      \end{subfigure}
% %      \hfill
% %      \begin{subfigure}[b]{0.48\textwidth}
% %          \centering
% %          \includegraphics[width=\textwidth]{figure/redundant_feature_exp_10_feature/GPSHAP_std_BeeSwarm.png}
% %          \caption{GP-SHAP STD Beeswarm plot}
% %          \label{fig:three sin x}
% %      \end{subfigure}
% %     \caption{Examining the standard deviation of GP-SHAP values.}
% %     \label{fig:redundant_exp_10_feature_std}
% % \end{figure}

% % \subsection{Redundant feature case with 3 features}
% % We repeat the above experiment but with 3 features this time. We will examine closer and plot the Shapley values along with their uncertainty on the y-axis and their corresponding feature value on the x-axis.

% % \begin{figure}
% %     \centering
% %     \includegraphics[width=\textwidth]{figure/redundant_feature_exp_3_feature/SV_vs_X.png}
% %     \caption{Mean and std of Shapley values for each feature is plotted. We see that GPSHAP consistently gives close to 0 SVs to the redundant feature with high confidence. The histogram of the feature is plotted as well and we see that as we move away from high density region, the uncertainty increases.}
% %     \label{fig:SV_vs_X}
% % \end{figure}

% % \begin{figure}
% %     \centering
% %     \includegraphics[width=\textwidth]{figure/redundant_feature_exp_3_feature/Uncertainty_vs_X.png}
% %     \caption{Uncertainty does increase as expected when our feature point is at the low density region of the data distribution. This is what we should expect.}
% %     \label{fig:Uncertainty_vs_X}
% % \end{figure}

% % \subsection{Real world experiment on diabetes dataset}

% % Check out the attached HTML file for results.

% % \section{Discussion Points}

% % Here are a few questions that we should think about:
% % \begin{itemize}
% %     \item What experiments are we used to verify this uncertainty makes sense?
% %     \item What are some practical usage of such uncertainty? Can we use it to do BayesOpt in any sense? Use it to design a better acquisition function? to reduce search space if we know there are certain dimension in the feature space that is useless? 
% %     \item What is the best visualisation for this problem?
% %     \item Epistemic versus aleatoric uncertainty:
% %     \begin{itemize}
% %         \item I think the uncertainty captured in the SVs so far are all from the epistemic uncertainty. 
% %         \item It doesn't make sense to use aleatoric here at all right? Aleatoric uncertainties are the intrinsic uncertainty exists that aren't contributed by the covariates?
% %     \end{itemize}
% % \end{itemize}

% % \subsection{Competitors}
% % \begin{itemize}
% %     \item In order to do the same thing, one would need to sample solution paths from the posterior GP, and apply KernelSHAP on top, but that only works for interventional SVs, unless you estimate a conditional distribution $p(Y\mid X)$.
% %     \item BayesSHAP? Use their arguments on why probabilistic SHAP is good there? This thesis is an excellent source for reference: 
% %     \begin{itemize}
% %         \item https://scholarship.tricolib.brynmawr.edu/bitstream/handle/10066/23538/2021LiR.pdf?sequence=1&isAllowed=y
% %     \end{itemize}
% % \end{itemize}
